ES Attack: Model Stealing against Deep Neural Networks without Data Hurdles

Deep neural networks (DNNs) have become the essential components for various commercialized machine learning services, such as Machine Learning as a Service (MLaaS). Recent studies show that machine learning services face severe privacy threats - well-trained DNNs owned by MLaaS providers can be stolen through public APIs, namely model stealing attacks. However, most existing works undervalued the impact of such attacks, where a successful attack has to acquire confidential training data or auxiliary data regarding the victim DNN. In this paper, we propose ES Attack, a novel model stealing attack without any data hurdles. By using heuristically generated synthetic data, ES Attack iteratively trains a substitute model and eventually achieves a functionally equivalent copy of the victim DNN. The experimental results reveal the severity of ES Attack: i) ES Attack successfully steals the victim model without data hurdles, and ES Attack even outperforms most existing model stealing attacks using auxiliary data in terms of model accuracy; ii) most countermeasures are ineffective in defending ES Attack; iii) ES Attack facilitates further attacks relying on the stolen model.

==> bio.tex <==

% \vskip -2.5\baselineskip plus -1fil
% \vspace{-2em}
\begin{IEEEbiography}[{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{bio_fig/Xiaoyong-Yuan_rsz.png}}]{Xiaoyong (Brian) Yuan} received the B.S. degree from Fudan University, Shanghai, China, in 2012, the M.E. degree from Peking University, Beijing, China, in 2015, and the Ph.D degree from University of Florida, Gainesville, FL, in 2020. 

Dr. Yuan is an assistant professor at the College of Computing, Michigan Technological University, Houghton, MI. His research interest mainly spans the fields of machine learning, deep learning, security and privacy, and cloud computing.
\end{IEEEbiography}


\begin{IEEEbiography}[{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{bio_fig/LeahDing.jpg}}]{Leah Ding} received the Ph.D. degree in Electrical Engineering from the University at Buffalo in 2013. She is currently an Associate Professor with the Department of Computer Science, American University, Washington D.C. Her research interests include cyber security, machine learning, wireless and emerging networks.
\end{IEEEbiography}
% \vspace{-2em}
% \vskip -2.5\baselineskip plus -1fil

\begin{IEEEbiography}[{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{bio_fig/zhang}}]{Lan Zhang} received the B.S. degree and M.S. degree from the University of Electronic Science and Technology of China in 2013 and 2016, respectively, and the Ph.D. degree from the University of Florida in 2020. 

Dr. Zhang is an assistant professor in the Department of Electrical and Computer Engineering at Michigan Technological University, Houghton, MI. Her research interest mainly spans wireless communications and distributed machine learning in various cyber-physical systems and Internet of Things applications.
\end{IEEEbiography}
% \vspace{-2em}

\begin{IEEEbiography}[{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{bio_fig/andyli.png}}]{Xiaolin (Andy) Li} received the Ph.D. degree in computer engineering from Rutgers University, New Brunswick, NJ, USA.

Dr. Li is Partner of Tongdun Technology, heading the AI Institute; Chair Professor and Chief Scientist of IBMC, Chinese Academy of Sciences. He was a Professor at the University of Florida and founding center director of NSF Center for Big Learning. His research interests include deep learning, cloud computing, security \& privacy, IoT, and intelligent medicine.
\end{IEEEbiography}

\begin{IEEEbiography}[{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{bio_fig/wu}}]{Dapeng Oliver Wu} (S'98--M'04--SM’06--F'13)  received a Ph.D. degree in electrical and computer engineering from Carnegie Mellon University, Pittsburgh, PA, in 2003. He is a professor at the Department of Electrical and Computer Engineering, University of Florida, Gainesville, FL and the director of NSF Center for Big Learning.  His research interests are in the areas of networking, communications, signal processing, computer vision, machine learning, smart grid, and information and network security. He received University of Florida Term Professorship Award in 2017, University of Florida Research Foundation Professorship Award in 2009, AFOSR Young Investigator Program (YIP) Award in 2009, ONR Young Investigator Program (YIP) Award in 2008, NSF CAREER award in 2007, the IEEE Circuits and Systems for Video Technology (CSVT) Transactions Best Paper Award for Year 2001, and the Best Paper Awards in IEEE GLOBECOM 2011 and International Conference on Quality of Service in Heterogeneous Wired/Wireless Networks (QShine) 2006.

He has served as Editor in Chief of IEEE Transactions on Network Science and Engineering, Editor-at-Large for IEEE Open Journal of the Communications Society, founding Editor-in-Chief of Journal of Advances in Multimedia, and Associate Editor for IEEE Transactions on Cloud Computing, IEEE Transactions on Communications, IEEE Transactions on Signal and Information Processing over Networks, IEEE Signal Processing Magazine, IEEE Transactions on Circuits and Systems for Video Technology, IEEE Transactions on Wireless Communications and IEEE Transactions on Vehicular Technology.
\end{IEEEbiography}
